The Halo Bispectrum Multipoles in Redshift Space

We present the analysis of the halo bispectrum in redshift-space in terms of its multipoles, monopole, quadrupole and hexadecapole, measured from a large set of simulations. We fit such measurements with a tree-level model in perturbation theory that depends on linear and nonlinear bias parameters as well as on the growth rate $f$ of density fluctuations. The likelihood analysis takes advantage of a very large set of mock catalogs, enabling a robust estimation of the covariance properties for all multipoles. We compare the numerical estimate of the covariance matrix to its Gaussian prediction finding discrepancies of 10% or less for all configurations with the sole exception of the squeezed triangles in the monopole case. We find the range of validity of the tree-level model, for the total simulation volume of about 1000 $h^{-3}\, {\rm Gpc}^3$, reaches a maximum wavenumber of $0.08 \, h \, {\rm Mpc}^{-1}$ for the monopole, while it is limited to $0.06$ and $0.045\, h \, \rm{Mpc}^{-1}$ respectively for quadrupole and hexadecapole. Despite this, the addition of the quadrupole to the analysis allows for significant improvements on the determination of the model parameters and specifically on $f$, similarly to the power spectrum case. Finally, we compare our numerical estimate for the full covariance with its theoretical prediction in the Gaussian approximation and find the latter to work remarkably well in the context of simulation boxes with periodic boundary condition.

==> extra_on_multipoles_binning.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analytical evaluation of the bispectrum multipoles}
\label{app:A}

The orientation of the $\left\{\kv_1, \kv_2, \kv_3\right\}$ triangle w.r.t. the LOS in the model for the redshift-space bispectrum $B_s(\kv_1, \kv_2, \kv_3,\hat{n})$, eq.(\ref{eq:Btheory}), is expressed entirely in terms of products of powers of the cosines $\mu_i\equiv \hat{k}_i\cdot\hat{n}$ that can be factorised in each contribution.

%To compute the multipoles in equation (3) it is convenient to note that:
%\begin{itemize}
%    \item the dependence on $\mu_1$ is only in $\mu_2$ and $\mu_3$
%    \be
%    \mu_2 = \mu_1\mu_{12}-\sqrt{1-\mu_1^2}\sqrt{1-\mu^2_{12}}\cos(\xi)
%    \ee
%    \be
%    \mu_3 = \frac{\textbf{k}_3\cdot\hat{n}}{k_3} =- \frac{k_1\mu_1 + k_2\mu_2}{k_3}
%    \ee
%    \item $\xi$ enters only in $\mu_2$ and $\mu_3$
%    \
%\end{itemize}
%In this way, equation (3) can be written as sum of terms which show integrands that are a combination of $\mu_1$, $\mu_2$ and $\mu_3$. It is helpful to give a naming these terms $\mathcal{I}_{\alpha \beta \gamma}$:

The integrals defining the bispectrum multipoles in eq.~(\ref{e:Blm}) are therefore limited to integrals of such combinations, with the additional factor given by the spherical harmonics, or, in the $m=0$ case, Legendre polynomials (these corresponding to additional powers of $\mu_1$). We denote these integrals as  
\be
\mathcal{I}_{\alpha \beta \gamma} = \int_{-1}^{+1} d\mu_1 \int_{0}^{2\pi} d\xi\, \mu_1^{\alpha}\,\mu_2^{\beta}(\mu_1, \xi)\,\mu_3^{\gamma}(\mu_1, \xi)\,.
\ee
where
\be
\mu_2(\mu_1,\xi) = \mu_1\mu_{12}-\sqrt{1-\mu_1^2}\sqrt{1-\mu^2_{12}}\cos\xi
\ee
and 
\be
\mu_3(\mu_1,\xi) = - \frac{k_1\mu_1 + k_2\mu_2(\mu_1,\xi)}{k_3}\,,
\ee
having introduced $\mu_{12} \equiv \hat{k}_1\cdot\hat{k_2}$.

\emi{We could maybe derive some properties for these integrals that can shorten the list below} They are explicitly given by
\begin{align}
\mathcal{I}_{000} & =   4\pi \\
\mathcal{I}_{200} & =  \mathcal{I}_{020} = \frac{4\pi}{3}\\
%\mathcal{I}_{020} & = & \frac{4\pi}{3}\\
\mathcal{I}_{002} & =  \frac{4\pi}{3}\frac{k_1^2+k_2^2+2k_1k_2\sqrt{1+S_{2, 12}}}{k_3^2}\\
\mathcal{I}_{101} & =  -\frac{4\pi}{3}\frac{k_1+k_2\sqrt{1+S_{2,12}}}{k_3}\\
\mathcal{I}_{110} & =  \frac{4\pi}{3}\sqrt{1+S_{2, 12}}\\
\mathcal{I}_{011} & =  -\frac{4\pi}{3}\frac{k_2+k_1\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{220} & =  \frac{4\pi}{5}+\frac{8\pi S_{2, 12}}{15} \\
\mathcal{I}_{202} & = \frac{4\pi}{5}\frac{k_1^2+k_2^2+2k_1k_2\sqrt{1+S_{2, 12}}}{k_3^2}+\frac{8\pi k_2^2 S_{2, 12}}{15 k_3^2}\\
\mathcal{I}_{022} & = \frac{4\pi}{5}\frac{k_1^2+k_2^2+2 k_1 k_2\sqrt{1+S_{2, 12}}}{k_3^2}+\frac{8\pi k_1^2S_{2, 12}}{15 k_3^2}\\
\mathcal{I}_{301} & = -\frac{4\pi}{5}\frac{k_1+k_2\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{031} & =  -\frac{4\pi}{5}\frac{k_2+k_1\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{310} & =  \frac{4\pi}{5}\sqrt{1+S_{2, 12}}\\
\mathcal{I}_{013} & =  -\frac{4\pi}{5}\frac{k_2^3+3 k_1^2 k_2+ 2k_1^2 k_2 S_{2, 12}+k_1^3\sqrt{1+S_{2, 12}}+ 3k_1 k_2^2\sqrt{1+S_{2, 12}}}{k_3^3}\\
\mathcal{I}_{130} & =  \frac{4\pi}{5}\sqrt{1+S_{2, 12}}\\
\mathcal{I}_{103} & =  -\frac{4\pi}{5}\frac{k_1^3+3 k_1 k_2^2 + 2 k_1 k_2^2 S_{2, 12} + k_2^3\sqrt{1+S_{2, 12}}+ 3k_1^2 k_2\sqrt{1+S_{2, 12}}}{k_3^3}\\
\mathcal{I}_{121} & =  -\frac{4\pi}{15}\frac{3 k_1+2k_1 S_{2, 12}+ 3 k_2\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{211} & =  -\frac{4\pi}{15}\frac{3k_2+2k_2 S_{2, 12}+ 3k_1\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{112} & =  \frac{4\pi}{15}\frac{6k_1 k_2+4k_1 k_2 S_{2, 12}+ 3k_1^2\sqrt{1+S_{2, 12}}+ 3k_2^2\sqrt{1+S_{2, 12}}}{k_3^2} \\
\mathcal{I}_{222} & =  \frac{4\pi}{35}\frac{2k_1 k_2\sqrt{1+S_{2,12}}(5+2S_{2, 12})+ k_1^2(5+4S_{2, 12})+k_2^2(5+4S_{2, 12})}{k_3^2}\\
\mathcal{I}_{141} & =  -\frac{4\pi}{35}\frac{5 k_1 + 4k_1S_{2, 12}+ 5k_2\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{411} & =  -\frac{4\pi}{35}\frac{5 k_2+4k_2 S_{2, 12}+5k_1\sqrt{1+S_{2, 12}}}{k_3}\\
\mathcal{I}_{114} & =  \frac{4\pi}{35}\frac{1}{k_3^4}\left[5 k_1^4\sqrt{1+S_{2, 12}}+5k_2^4\sqrt{1+S_{2, 12}}+6k_1^2 k_2^2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})
\right.\nn\\ & \left.
+4k_1^3 k_2(5+4S_{2, 12})+4 k_1 k_2^3(5+4S_{2, 12})\right]\\
\mathcal{I}_{123} & =  -\frac{4\pi}{35}\frac{1}{k_3^3}\left[5k_2^3\sqrt{1+S_{2, 12}}+3k_1^2 k_2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+
\right.\nn\\ & \left.
+ k_1^3(5+4S_{2, 12})+3k_1 k_2^2(5+4S_{2, 12})\right]\\
\mathcal{I}_{132} & =  \frac{4\pi}{35}\frac{5k_2^2\sqrt{1+S_{2, 12}}+ k_1^2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+2k_1 k_2 (5+4S_{2, 12})}{k_3^2}\\
\mathcal{I}_{312} & =  \frac{4\pi}{35}\frac{5 k_1^2\sqrt{1+S_{2, 12}}+ k_2^2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+ 2 k_1 k_2(5+4S_{2, 12})}{k_3^2}\\
\mathcal{I}_{213} & =  -\frac{4\pi}{35}\frac{1}{k_3^3}\left[5k_1^3\sqrt{1+S_{2, 12}}+3k_1 k_2^2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+
\right.\nn\\ & \left. 
3k_1^2 k_2(5+4S_{2, 12})+k_2^3(5+4S_{2, 12})\right]\\
\mathcal{I}_{321} & =  -\frac{4\pi}{35}\frac{k_2\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+k_1(5+4S_{2, 12})}{k_3}\\
\mathcal{I}_{231} & =  -\frac{4\pi}{35}\frac{k_1\sqrt{1+S_{2, 12}}(5+2S_{2, 12})+k_2(5+4S_{2, 12})}{k_3}\\
\mathcal{I}_{341} & = -\frac{4\pi}{315}\frac{5k_2\sqrt{1+S_{2, 12}}(7+4S_{2, 12})+k_1(35+40S_{2, 12}+8S^2_{2, 12})}{k_3}\\
\mathcal{I}_{431} & = -\frac{4\pi}{315}\frac{5k_1\sqrt{1+S_{2, 12}}(7+4S_{2, 12})+k_2(35+40S_{2, 12}+8S^2_{2, 12})}{k_3}\\
\mathcal{I}_{314} & = \frac{4\pi}{315}\frac{1}{k_3^4}\left[35k_1^4\sqrt{1+S_{2, 12}}+30k_1^2k_2^2\sqrt{1+S_{2, 12}}(7+4S_{2, 12})+\right.\nn\\
& \left. + 5k_2^4\sqrt{1+S_{2, 12}}(7+4S_{2, 12}) + 20k_1^3 k_2(7+6S_{2, 12})+4k_1 k_2^3(35+40S_{2, 12}+8S^2_{2, 12})\right]\\
\mathcal{I}_{413} & = -\frac{4\pi}{315}\frac1{k_3^3}\left[35 k_1^3\sqrt{1+S_{2, 12}}+15k_1 k_2^2 \sqrt{1+S_{2, 12}}(7+4S_{2, 12})+
\right.\nn\\ & \left.
+15k_1^2 k_2(7+6S_{2, 12})+k_2^3(35+40S_{2, 12}+8S^2_{2, 12})\right]
\\
\mathcal{I}_{134} & = \frac{4\pi}{315}\frac{1}{k_3^4}\left[35k_2^4\sqrt{1+S_{2, 12}}+30k_1^2k_2^2\sqrt{1+S_{2, 12}}(7+4S_{2, 12})+
\right.\nn\\ & \left.
+5k_1^4\sqrt{1+S_{2, 12}}(7+4S_{2, 12}) + 20 k_1 k_2^3(7+6S_{2, 12})+4 k_1^3 k_2 (35+40S_{2, 12}+8S^2_{2, 12})\right]
\\
\mathcal{I}_{143} & = 
-\frac{4\pi}{315}\frac{1}{k_3^3}\left[35 k_2^3\sqrt{1+S_{2, 12}}+15k_1^2 k_2 \sqrt{1+S_{2, 12}}(7+4S_{2, 12})+15k_1 k_2^2(7+6S_{2, 12})+
\right.\nn\\ & \left.
+ k_1^3(35+40S_{2, 12}+8S^2_{2, 12})\right]\,.
\end{align}

\emi{In fact, if the angle integration is equivalent (as it should) to a generic integration over all orientations, I would expect this to be true:}
\blue{
\be
\I_{\alpha,\beta,\gamma}(k_1,k_2,k_3)=\I_{\sigma(\alpha,\beta,\gamma)}[\sigma(k_1,k_2,k_3)]\,,
\ee
where $\sigma(...)$ represents a generic permutations of its arguments. \footnote{Notice that in general is not true that $\I_{\alpha,\beta,\gamma}(k_1,k_2,k_3)=\I_{\sigma(\alpha,\beta,\gamma)}(k_1,k_2,k_3)$, so if we write, e.g.,  $\I_{200}+\I_{020}$ we implicitly mean $\I_{200}(k_1,k_2,k_3)+\I_{020}(k_1,k_2,k_3)$ and this is the sum of two different things.} If this is so, and if $S_{2,12}=-\sin^2 \theta_{12}=\mu^2_{12}-1$ (I couldn't find the definition), then we can simplify the integrals as follows}
\emi{Maybe I am finding different results, but mine satisfy the property above ...}
\blue{
\begin{align}
\I_{000} & =   4\pi \,,\\
\I_{200} & =  \I_{020} = \I_{002} =\frac{4\pi}{3}\,,\\
\I_{110} & =  \frac{2\pi}{3}\frac{k_1^2+k_2^2-k_3^2}{k_2\,k_1}\,,\\
\I_{220} & = \frac{2\pi}{15}\frac{ k_3^4 + k_2^4+ k_1^4 + 4 k_2^2 k_1^2  - 
   2 k_3^2 (k_2^2 + k_1^2)}{k_2^2 k_1^2}\,,\\
\I_{211} & = \frac{2\pi}{15}\frac{2 k_1^4 -  (k_2^2 - k_3^2)^2 - 
    k_1^2 (k_2^2 + k_3^2)}{k_1^2 k_2 k_3}\,,\\
\I_{310} & = \frac{2\pi}{5}\frac{k_3^2-k_1^2 - k_2^2}{k_1 k_2}\,,\\
\I_{400} & = \frac{4\pi}{5}\,,\\
\I_{222} & = \frac{2\pi}{35} \frac{k_1^6 - k_1^4 (k_2^2 + k_3^2) + (k_2^2 - k_3^2)^2 (k_2^2 + k_3^2) - k_1^2 (k_2^4 - 4 k_2^2 k_3^2 + k_3^4)}{k_1^2 k_2^2 k_3^2}\,,\\
\I_{321} & = -\frac{\pi}{35}\frac{3 k_1^6 + k_1^4 (3 k_2^2 - 5 k_3^2) - (k_2^2 - k_3^2)^3 + k_1^2 (-5 k_2^4 + 4 k_2^2 k_3^2 + k_3^4)}{k_1^3 k_2^2 k_3}\,,\\
\I_{330} & = -\frac{\pi}{35}\frac{(k_1^2 + k_2^2 - k_3^2) (k_1^4 + 
    k_1^2 (8 k_2^2 - 2 k_3^2) + (k_2^2 - k_3^2)^2)}{k_1^3 k_2^3}\,,\\
\I_{411} & = \frac{2\pi}{35}\frac{3 k1^4 - 2 (k_2^2 - k_3^2)^2 - 
   k_1^2 (k_2^2 + k_3^2)}{k_1^2 k_2 k_3}\,,\\
\I_{420} & = \frac{4\pi}{35}\frac{k_1^4 + 
   k_1^2 (3 k_2^2 - 2 k_3^2) + (k_2^2 - k_3^2)^2}{k_1^2 k_2^2}\,,\\
\I_{510} & = \frac{2\pi}{7}\frac{k_3^2-k_1^2 - k_2^2}{k_1 k_2}\,,\\
\I_{422} & = \frac{2\pi}{315}\frac{1}{k_1^4 k_2^2 k_3^2}\left[6 k_1^8 + (k_2^2 - k_3^2)^4 -  4 k_1^6 (k_2^2 + k_3^2) + 6 k_1^2 (k_2^2 - k_3^2)^2 (k_2^2 + k_3^2)
\right. \nn\\ & \left. 
- 3 k_1^4 (3 k_2^4 - 8 k_2^2 k_3^2 + 3 k_3^4)\right]\,,\\
\I_{431} & = \frac{2\pi}{315}\frac{1}{k_1^4 k_2^3 k_3}\left[4 k_1^8 + 
   k_1^6 (14 k_2^2 - 11 k_3^2) - (k_2^2 - k_3^2)^4 - k_1^2 (k_2^2 - k_3^2)^2 (11 k_2^2 + k_3^2)
   \right.\nn \\ & \left.
    + k_1^4 (-6 k_2^4 - 9 k_2^2 k_3^2 + 9 k_3^4)\right]\,,\\
\I_{521} & = -\frac{2\pi}{63}\frac{2 k_1^6 + k_1^4 (2 k_2^2 - 3 k_3^2) - (k_2^2 - k_3^2)^3 - 3 k_1^2 (k_2^4 - k_2^2 k_3^2)}{k_1^3 k_2^2 k_3}\,,\\
\I_{611} & = -\frac{2\pi}{63}\frac{4 k_1^4 - 3 (k_2^2 - k_3^2)^2 -  k_1^2 (k_2^2 + k_3^2)}{k_1^2 k_2 k_3}\,,\\
\I_{433} & =\frac{\pi}{231}\frac{1}{k_1^4 k_2^3 k_3^3}
\left[(2 k_1^{10} - 
2 k_1^8 (k_2^2 + k_3^2) - (k_2^2 - k_3^2)^4 (k_2^2 + k_3^2) + k_1^6 (-5 k_2^4 + 16 k_2^2 k_3^2 - 5 k_3^4)
\right.\nn \\ & \left.
- k_1^2 (k_2^2 - k_3^2)^2 (k_2^4 + 10 k_2^2 k_3^2 + k_3^4) +  k_1^4 (7 k_2^6 - 9 k_2^4 k_3^2 - 9 k_2^2 k_3^4 + 7 k_3^6)) \right]
\,,\\
\I_{541} & = - \frac{\pi}{693}\frac{1}{k_1^5 k_2^4 k_3}
\left[5 k_1^{10} + k_1^8 (35 k_2^2 - 19 k_3^2) - (k_2^2 - k_3^2)^5 - k_1^2 (k_2^2 - k_3^2)^3 (19 k_2^2 + k_3^2) + 
\right.\nn \\ & \left.
k_1^6 (20 k_2^4 - 64 k_2^2 k_3^2 + 26 k_3^4) - 2 k_1^4 (20 k_2^6 - 18 k_2^4 k_3^2 - 9 k_2^2 k_3^4 + 7 k_3^6) \right]\,,\\
\I_{631} & = \frac{\pi}{231}\frac{1}{k_1^4 k_2^3 k_3}
\left[ 5 k1^8 + k1^6 (15 k2^2 - 13 k3^2) - 2 (k2^2 - k3^2)^4 
\right.\nn \\ & \left.
- k1^2 (k2^2 - k3^2)^2 (13 k2^2 - k3^2) + k1^4 (-5 k2^4 - 8 k2^2 k3^2 + 9 k3^4)\right]
\,.
\end{align}
}

We can group all contributions to the bispectrum multipoles according to the source of quadratic nonlinearity, that is \emi{What Scoccimarro (2013) reference did you mean, Fede?}
\be
B_\ell(k_1,k_2,k_3) =   B_{\ell}^{(F_2)}+B_{\ell}^{(b_2)} + B_{\ell}^{(S_2)} + B_{\ell}^{(G_2)} + B_{\ell}^{({\rm mixed})}\,.
\ee
These contributions can be expressed in terms of the $\I_{\alpha\beta\gamma}$. In the monopole case we have
\small{
\begin{align}
%%% 0, b2 %%%
B_{0}^{(b2)} & = 
\frac{b_1^2 b_2}{2\sqrt{\pi}}\,\I_{000}\, \Big[ P_L(k_1)\,P_L(k_2)+2~{\rm perm.} \Big]
+ \nn \\ &
+ \frac{b_1 b_2 f}{2\sqrt{\pi}}\Big[(\I_{200}+\I_{020})P_L(k_1)P_L(k_2)+(\I_{200}+\I_{002})P_L(k_1)P_L(k_3)+ (\I_{020}+\I_{002})P_L(k_2)P_L(k_3) \Big]
+ \nn \\ &
+ \frac{b_2 f^2}{2\sqrt{\pi}} \Big[ \I_{220}P_L(k_1) P_L(k_2) + \I_{202} P_L(k_1) P_L(k_3) + \I_{022}P_L(k_2) P_L(k_3) \Big]
\,, \\ 
%%% 0, F2 %%%
B_{0}^{(F_2)} & = 
\frac{b_1^3}{\sqrt{\pi}}\I_{000}\Big[F_2(k_1, k_2;k_3) P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big]
+ \nn \\ &
+ \frac{b_1^2 f}{\sqrt{\pi}} \Big[(\I_{200}+\I_{020})F_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + (\I_{200} + \I_{002}) F_2(k_1, k_3; k_2) P_L(k_1) P_L(k_3)
+ \nn \\ & 
+(\I_{020}+\I_{002})F_2(k_2, k_3; k_1)P_L(k_2)P_L(k_3)\Big] + 
 \nn \\ & 
 + \frac{b_1 f^2}{\sqrt{\pi}} \Big[ \I_{220}F_2(k_1, k_2; k_3)P_L(k_1)P_L(k_2)+\I_{202}F_2(k_1, k_3; k_2)P_L(k_1)P_L(k_3) + 
 \nn \\ &
 + \I_{022} F_2(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big]
\,, \\
%%% 0, S2 %%%
B_{0}^{(S_2)} & = 
\frac{b_1^2 \bGt}{\sqrt{\pi}} \I_{000} \Big[ S(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + S(k_1, k_3; k_2) P_L(k_1) P_L(k_3) + S(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big]
+ \nn \\ &
+ \frac{b_1 \bGt f}{\sqrt{\pi}} \Big[ (\I_{200} + \I_{020}) S(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + (\I_{200} + \I_{002}) S(k_1, k_3; k_2) P_L(k_1) P_L(k_3) 
+ \nn \\ &
+ (\I_{020} + \I_{002}) S(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big] 
+ \nn \\ &
+ \frac{\bGt}{\sqrt{\pi} f^2} \Big[ \I_{220} S(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + \I_{202} S(k_1, k_3; k_2) P_L(k_1) P_L(k_3) 
+ \nn \\ &
+ \I_{022} S(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big]
\,, \\
%%% 0, G2 %%%
B_{0}^{(G_2)} & = 
\frac{b_1^2 f}{\sqrt{\pi}} \Big[\I_{002} G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + \I_{020} G_2(k_1, k_3; k_2) P_L(k_1) P_L(k_3) 
+ \nn \\ & 
+ \I_{200} G_2(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big] + 
\nn \\ & + \frac{b_1 f^2}{\sqrt{\pi}} \Big[ (\I_{202} + \I_{022})G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + (\I_{220} + \I_{022})G_2(k_1, k_3; k_2) P_L(k_1) P_L(k_3)
+ \nn \\ & 
+ (\I_{220}+\I_{202})G_2(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big] 
+ \nn \\ & 
+ \frac{f^3}{\sqrt{\pi}} \I_{222} \Big[ G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + G_2(k_1, k_3; k_2) P_L(k_1) P_L(k_3) 
+ \nn \\ & 
+ G_2(k_2, k_3; k_1) P_L(k_2) P_L(k_3) \Big]
\,, \\
%%% 0, mixed %%%
B_{0}^{(\text{mixed})} & = 
- \frac{b_1^3 f}{2\sqrt{\pi}} \Big[ \Big(\frac{k_3}{k_1}\I_{101}+\frac{k_3}{k_2}\I_{011}\Big) P_L(k_1) P_L(k_2) + \Big(\frac{k_2}{k_1}\I_{110}+\frac{k_2}{k_3}\I_{011}\Big) P_L(k_1) P_L(k_3)
+ \nn \\ & 
+\Big(\frac{k_1}{k_2}\I_{110}+\frac{k_1}{k_3}\I_{101}\Big) P_L(k_2) P_L(k_3)\Big] 
+ \nn \\ &
- \frac{b_1^2 f^2}{2\sqrt{\pi}}\Big[\Big(\frac{k_3}{k_1}(\I_{301} + 2 \I_{121})+\frac{k_3}{k_2}(\I_{031}+2\I_{211})\Big) P_L(k_1) P_L(k_2) 
+ \nn \\ &
+ \Big(\frac{k_2}{k_1}(\I_{310}+2\I_{112})+\frac{k_2}{k_3}(\I_{013} + 2 \I_{211})\Big) P_L(k_1) P_L(k_3)
+ \nn \\ &
+ \Big(\frac{k_1}{k_2}(\I_{130}+2\I_{112})+\frac{k_1}{k_3}(\I_{103} + 2 \I_{121})\Big) P_L(k_2) P_L(k_3) \Big] 
+ \nn \\ &
- \frac{b_1 f^3}{2\sqrt{\pi}}\Big[\Big(\frac{k_3}{k_1}(\I_{141}+2 \I_{321})+ \frac{k_3}{k_2}(\I_{411}+2\I_{231})\Big) P_L(k_1) P_L(k_2) 
+ \nn \\ &
+ \Big(\frac{k_2}{k_1}(\I_{114}+ 2\I_{312}) + \frac{k_2}{k_3}(\I_{411}+2\I_{213}) \Big) P_L(k_1) P_L(k_3) 
+ \nn \\ &
+ \Big(\frac{k_1}{k_2}(\I_{114}+2\I_{132}) + \frac{k_1}{k_3}(\I_{141}+2\I_{123})\Big) P_L(k_2) P_L(k_3)\Big]
+ \nn \\ & 
- \frac{f^4}{2\sqrt{\pi}}\Big[\Big(\frac{k_3}{k_1}\I_{341} + \frac{k_3}{k_2}\I_{431}\Big) P_L(k_1) P_L(k_2) + \Big(\frac{k_2}{k_1}\I_{314} + \frac{k_2}{k_3}\I_{413}\Big) P_L(k_1) P_L(k_3) 
+ \nn \\ & 
+\Big(\frac{k_1}{k_2}\I_{134} + \frac{k_1}{k_3}\I_{143}\Big) P_L(k_2) P_L(k_3) \Big]
\end{align}
}

\blue{We can rewrite the equations above as below, with the ``2~perm.'' acting as well on the $\I_{\alpha\beta\gamma}$ indices 
\begin{align}
%%% 0, F2 %%%
\label{e:B0F2}
B_{0}^{(F_2)} & = 
\frac{b_1^3}{\sqrt{\pi}}\I_{000} \Big[ F_2(k_1, k_2;k_3) P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big]
+ \nn\\ & 
+ \frac{b_1^2 f}{\sqrt{\pi}} \Big[(\I_{200}+\I_{020})F_2(k_1, k_2; k_3)P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big] 
+ \nn \\ & 
+ \frac{b_1 f^2}{\sqrt{\pi}} \Big[\I_{220}F_2(k_1, k_2; k_3)P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big]
\,, \\
%%% 0, b2 %%%
\label{e:B0B2}
B_{0}^{(b2)} & = 
\frac{b_1^2 b_2}{2\sqrt{\pi}}\,\I_{000}\,\Big[P_L(k_1)P_L(k_2)+2~{\rm perm.}\Big]
+ \nn \\ & 
+ \frac{b_1 b_2 f}{2\sqrt{\pi}}\Big[(\I_{200}+\I_{020}) P_L(k_1) P_L(k_2) + 2~{\rm perm.}]
+ \nn \\ &
+ \frac{b_2 f^2}{2\sqrt{\pi}} \Big[ \I_{220}P_L(k_1) P_L(k_2) +2~{\rm perm.} \Big] 
\,, \\ 
%%% 0, S2 %%%
\label{e:B0S2}
B_{0}^{(S_2)} & = 
\frac{b_1^2 \bGt}{\sqrt{\pi}} \I_{000} \Big[ S(k_1, k_2; k_3)P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big] 
+ \nn \\ & 
+ \frac{b_1 \bGt f}{\sqrt{\pi}} \Big[ (\I_{200}+ \I_{020})S(k_1, k_2; k_3)P_L(k_1)P_L(k_2)+2~{\rm perm.} \Big]
+ \nn \\ & 
+ \frac{\bGt f^2}{\sqrt{\pi}} \Big[ \I_{220} S(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + 2~{\rm perm.} \Big]
\,, \\
%%% 0, G2 %%%
\label{e:B0G2}
B_{0}^{(G_2)} & = 
\frac{b_1^2 f}{\sqrt{\pi}} [\I_{002} G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + 2~{\rm perm.} ] 
+ \nn \\ & 
+ \frac{b_1 f^2}{\sqrt{\pi}} \Big[ (\I_{202} + \I_{022})G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2) + 2~{\rm perm.} \Big] 
+ \nn \\ & 
+ \frac{f^3}{\sqrt{\pi}} \I_{222} \Big[ G_2(k_1, k_2; k_3) P_L(k_1) P_L(k_2)+ 2~{\rm perm.} \Big]
\,, \\
%%% 0, Mixed %%%
\label{e:B0Mixed}
B_{0}^{(\text{mixed})} & = 
- \frac{b_1^3 f}{2\sqrt{\pi}}\Big[\Big(\frac{k_3}{k_1}\I_{101}+\frac{k_3}{k_2}\I_{011}\Big)P_L(k_1)P_L(k_2) +2~{\rm perm.}] 
- \nn \\ & 
-\frac{b_1^2 f^2}{2\sqrt{\pi}}\Big[\Big(\frac{k_3}{k_1}(\I_{301} + 2\I_{121})+\frac{k_3}{k_2}(\I_{031}+2\I_{211})\Big)P_L(k_1)P_L(k_2) + 2~{\rm perm.}\Big] 
- \nn \\ & 
- \frac{b_1 f^3}{2\sqrt{\pi}} \Big[\Big(\frac{k_3}{k_1}(\I_{141}+2 \I_{321})+ \frac{k_3}{k_2}(\I_{411}+2\I_{231})\Big)P_L(k_1)P_L(k_2) + 2~{\rm perm.}\Big]
- \nn \\ & 
- \frac{f^4}{2\sqrt{\pi}} \Big[\Big(\frac{k_3}{k_1}\I_{341} + \frac{k_3}{k_2}\I_{431}\Big)P_L(k_1) P_L(k_2)+2~{\rm perm.}\Big]
\,.
\end{align}
}

The shot noise of the monopole is modeled according to:
\begin{align}
B_{0}^{(\text{shot-noise})}  = \frac{1}{2\sqrt{\pi}}\Big\{ \frac{1}{(2\pi)^3 \tilde{n}}\Big[ & b_1^2\,\I_{000}\,\Big(P_L(k_1)+ P_L(k_2) + P_L(k_3)\Big) \nn \\
&  + b_1 f\Big(\I_{200}P(k_1) + \I_{020}P(k_2)P +\I_{002}P(k_3) \Big) + \nn \\
&  + f^2\Big(\I_{400}P(k_1) + \I_{040}P(k_2)P +\I_{004}P(k_3) \Big)\Big] + \nn \\
& +\frac{\I_{000}}{(2\pi)^6\bar{n}^2}\Big\}
\end{align}
For the quadrupole and hexadecapole, equation (3) becomes:
\begin{align}
B_2(k_1, k_2, k_3) &= \int_{-1}^{+1}d\mu_1\int_0^{2\pi}d\xi B(k_1, k_2, k_2, \mu_1, \xi)\Big[\frac{1}{4}\sqrt{\frac{5}{\pi}}(3\mu_1^2 - 1)\Big]
\\
B_4(k_1, k_2, k_3) &= \int_{-1}^{+1}d\mu_1\int_0^{2\pi}d\xi B(k_1, k_2, k_2, \mu_1, \xi)\Big[\frac{3}{16}\sqrt{\frac{1}{\pi}}(35\mu_1^4 - 30\mu_1^2 + 3)\Big]
\end{align}
It is convenient to notice that, using this notation, the multipoles can be written quickly starting from equations (\ref{e:B0F2})-(\ref{e:B0Mixed}).
If we look at the quadrupole, for example, the first term bearing the $\mu_1^2$ contribution can be computed by replacing each $\I_{\alpha \beta \gamma}$ term with $\I_{\alpha +2 \beta \gamma}$ while the second term is analogous to the monopole. Similarly, for the hexadecapole, one can compute the contribution coming from the $\mu_1^4$ term by sending $\I_{\alpha \beta \gamma}$ to $\I_{\alpha+4 \beta \gamma}$.
The shot noise of the quadrupole term is
\begin{align}
B_{2}^{(\text{shot-noise})} & = \frac{1}{2}\sqrt{\frac{5}{\pi}}\Big\{ \frac{3}{(2\pi)^3 \tilde{n}}\Big[ b_1^2\Big(P(k_1)+ P(k_2) + P(k_3)\Big)\I_{200} \nn \\
& + b_1 f\Big(\I_{400}P(k_1) + \I_{420}P(k_2)P +\I_{402}P(k_3) \Big) + \nn \\
& + f^2\Big(\I_{600}P(k_1) + \I_{240}P(k_2)P +\I_{204}P(k_3) \Big)\Big]  +\frac{3\,\I_{200}}{(2\pi)^6\bar{n}^2}+ \nn\\
& - \frac{1}{(2\pi)^3 \tilde{n}}\Big[ b_1^2\Big(P(k_1)+ P(k_2) + P(k_3)\Big)\I_{000} \nn\\
& + b_1 f\Big(\I_{200}P(k_1) + \I_{020}P(k_2)P +\I_{002}P(k_3) \Big) + \nn\\
& + f^2\Big(\I_{400}P(k_1) + \I_{040}P(k_2)P +\I_{004}P(k_3) \Big)\Big]  -\frac{\I_{000}}{(2\pi)^6\bar{n}^2}\Big\} 
\end{align}

\emi{Everything without the $f$ factor in front should go to zero in the eq. above}

\emi{Maybe, we can introduce quantities like this:}
\blue{
\begin{align}
\J^{(2)}_{\alpha\beta\gamma} & \equiv \frac14\sqrt{\frac{5}{\pi}}\left(3\,\I_{\alpha+2\,\beta\,\gamma}-\I_{\alpha\,\beta\,\gamma}\right)\,\\
\J^{(4)}_{\alpha\beta\gamma} & \equiv \frac3{16\,\sqrt{\pi}}\left(35\,\I_{\alpha+4\,\beta\,\gamma}-30\I_{\alpha+2\,\beta\,\gamma}+3\I_{\alpha\,\beta\,\gamma}\right)\,.
\end{align}
This way we can keep the expressions written in terms of permutations of the lower indeces (although ,
\begin{align}
B_{\ell}^{(\text{shot-noise})} & =  \frac{2}{(2\pi)^3 \tilde{n}}\Big[ b_1 f\,\J^{(\ell)}_{200}\,P_L(k_1) + f^2\,\J^{(\ell)}_{400}\,P_L(k_1) + 2~{\rm perm.}\Big] \,,
\end{align}
since $\J^{(\ell)}_{000}=0$ (also $\J^{(4)}_{200}=0$). BTW, I am not sure about the factor of 2 in front of this last eq. Also ... do we have the $(2\pi)^3$ for our FT convention? I thought we used the other
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Considerations on the binning of the bispectrum multipoles}

\emi{This appendix should be removed I think, maybe save it somewhere}

Take the estimator for the bispectrum multipoles in redshift space
\be
\hat B_{\ell m}(k_1, k_2, k_3) = \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\delta_{\qv_1}^{(s)}\delta_{\qv_2}^{(s)}\delta_{\qv_3}^{(s)} Y_{\ell m}(\theta, \xi),
\ee
where both $\theta$ and $\xi$ are angles that are functions of the $\qv_1, \qv_2, \qv_3$. The theoretical model, then, can be consistently bin-averaged by replacing the product of the three deltas with the theoretical prediction of the anisotropic bispectrum,
\be
\hat B_{\ell m}^{\rm theory}(k_1, k_2, k_3) = \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})B^{(s)}_{\rm theory}(\qv_1, \qv_2, \qv_3) Y_{\ell m}(\theta, \xi).
\ee
Without any loss of generality, we can write the anisotropic bispectrum as the linear combination of the redshift-space multipoles,
\be
\hat B_{\ell m}^{\rm theory}(k_1, k_2, k_3) = \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\sum_{\ell ^\prime} \sum_{m^\prime} B_{\ell^\prime m^\prime}^{\rm theory}(q_1, q_2, q_3) Y_{\ell m}(\theta, \xi)Y_{\ell^\prime m^\prime}(\theta, \xi).
\ee
This allows to write the full bin-average of the bispectrum multipoles as a function of the multipoles themselves, that are independent from any angle, and depend only on the moduli of the $\qv_i$'s.

Notice that the theoretical prediction for the anisotropic bispectrum in equation 31 is actually defined over the full continuum Fourier space, since it is just a functional of the linear power spectrum and the SPT kernels in redshift space, that are already defined over the continuum. It is only when the model of the anisotropic bispectrum is multiplied by the spherical harmonics, and is then averaged over the discrete Fourier space, that discretization is having effect. This means that the theoretical predictions for the multipoles are as well defined on continuum Fourier space, and therefore they do not need to be further binned.

The predictions for the bispectrum multipoles can then be computed over continuous Fourier space, and thus integration in equation 3 can be performed analytically. The same is true for the $\mathcal I_{\alpha\beta\gamma}$ integrals in equation 12.

Now, following the equations in the main text, each multipole can be written as a linear combination of some $k_i$-dependent terms and some coefficients $\beta$, that are products of some of the model parameters (bias, growth rate, shot-noise parameters). Therefore,
\be
    B_{\ell m}(k_1, k_2, k_3) = \sum_{i=1}^{N_{\ell m}} \beta_i(\boldsymbol \theta) \mathcal B^i_{\ell m}(k_1, k_2, k_3).
\ee

This allows to write the bin-averaged theoretical prediction of the bispectrum multipoles conveniently as
\bea
\hat B_{\ell m}^{\rm theory}(k_1, k_2, k_3) &=& \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\sum_{\ell ^\prime} \sum_{m^\prime} \sum_{i=1}^{N_{\ell m}} \beta_i(\boldsymbol \theta) \mathcal \mathcal B^i_{\ell^\prime m^\prime} Y_{\ell m}(\theta, \xi)Y_{\ell^\prime m^\prime}(\theta, \xi) \nonumber \\
&=&\sum_{i=1}^{N_{\ell m}} \beta_i(\boldsymbol \theta)\frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\sum_{\ell ^\prime} \sum_{m^\prime} \mathcal B^i_{\ell^\prime m^\prime}(q_1, q_2, q_3) Y_{\ell m}(\theta, \xi)Y_{\ell^\prime m^\prime}(\theta, \xi) \nonumber,
\eea
and thus, by defining the bin-average of the $B^i_{\ell^\prime m^\prime}(q_1, q_2, q_3)$ as
\be
\hat {\mathcal B}^i_{\ell m}(k_1, k_2, k_3) = \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\sum_{\ell^\prime} \sum_{m^\prime} \mathcal {B} ^i_{\ell^\prime m^\prime}(q_1, q_2, q_3) Y_{\ell m}(\theta, \xi)Y_{\ell^\prime m^\prime}(\theta, \xi),
\ee
the full bin-average of the theoretical prediction becomes
\be
\hat B_{\ell m}^{\rm theory}(k_1, k_2, k_3) = \sum_{i=1}^{N_{\ell m}} \beta_i(\boldsymbol \theta)\hat {\mathcal B}^i_{\ell m}(k_1, k_2, k_3),
\ee
where, once the cosmology is fixed, the $\hat {\mathcal B}^i_{\ell m}(k_1, k_2, k_3)$ are computed only once, are tabulated, and are later linearly combined with the model parameters.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Further considerations on the binning of the bispectrum multipoles}


I copy from the PK notes some definitions explicitly accounting for a discrete Fourier grid (i.e. finite, periodic volume).


The Fourier transform of the density contrast is defined, in our convention, as
\be
\tilde{\delta}(\kv)  \equiv  \int_V d^3x\, e^{-i\kv\cdot\xv}\,\delta(\xv)\,,
\ee
with the inverse given by the series
\be
\del(\xv)  \equiv  \frac{k_f^3}{(2\pi)^3}\, \sum_{\kv}\,e^{i\kv\cdot\xv}\,\td(\kv)\,=  \frac{1}{V}\, \sum_{\kv}\,e^{i\kv\cdot\xv}\,\td(\kv)\,,
\ee
since $\kv$ is discretised in multiples of the fundamental frequency $k_{f}=2\pi/L$ in each spatial direction. We will always explicitly show the argument of each function in addition to identify Fourier-space objects with a tilde.\footnote{In this convention for the Fourier transform,  the Dirac delta in real space and the Kronecker delta in Fourier space are given, respectively by the following representations
\bdm
\del_D(\xv)=\frac1V\sum_{\kv} \,e^{i\,\kv\cdot\xv}\quad {\rm and} \quad \del^K_{\kv}=\frac1V\int d^3x\,e^{-i\,\kv\cdot\xv}\,.
\edm
}

The power spectrum $P(k)$ is then defined as the two-point function of $\del(\kv)$, that is
\be\label{eq:ps}
\langle \del(\kv_1)\,\del(\kv_2)\rangle \equiv (2\pi)^3\frac{\del^K_{\kv_{12}}}{k_f^3}\,P(k_1)=V\,\del^K_{\kv_{12}}\,P(k_1)\,,
\ee
with $\langle\, \dots\rangle$ representing the ensemble average, $\kv_{i_1,\dots,i_n}\equiv\kv_{i_1}+\dots+\kv_{i_n}$ and $\del^K_\kv$ being the Kronecker delta defined in such a way to be equal to 1 for a vanishing argument $\kv=0$, zero otherwise. Similarly, the bispectrum $B(k_1,k_2,k_3)$ is defined as 
\be
\langle \del(\kv_1)\,\del(\kv_2)\,\del(\kv_3)\rangle \equiv (2\pi)^3\,\frac{\del_{\kv_{123}}^K}{k_f^3}\,\,B(\kv_1,\kv_2,\kv_3)\,.
\ee
In this convention the continuous limit is recovered for $V\rightarrow \infty$ or $k_f\rightarrow 0$  with $\del^K_\kv/k_f^3\rightarrow \del_D(\kv)$, the latter being a Dirac delta function.  


The estimator for the bispectrum multipoles in redshift space is given by
\be
\hat B_{\ell m}(k_1, k_2, k_3) = \frac{1}{V}\frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\delta_{\qv_1}^{(s)}\delta_{\qv_2}^{(s)}\delta_{\qv_3}^{(s)} Y_{\ell m}(\theta, \xi),
\ee
where both angles $\theta$ and $\xi$ are functions of the $\qv_1, \qv_2, \qv_3$ and where
\be
N_B(k_1, k_2, k_3) = \sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\,.
\ee
We have then
\bea
\langle\hat B_{\ell m}(k_1, k_2, k_3)\rangle 
& = & \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\langle\delta_{\qv_1}^{(s)}\delta_{\qv_2}^{(s)}\delta_{\qv_3}^{(s)}\rangle Y_{\ell m}(\theta, \xi)\nn\\
& = & \frac{1}{N_B(k_1, k_2, k_3)}\sum_{\qv_1 \in k_1}\sum_{\qv_2 \in k_2}\sum_{\qv_3 \in k_3} \delta_K(\qv_{123})\,\frac{(2\pi)^3}{k_f^3}\,\,B(\qv_1,\qv_2,\qv_3) Y_{\ell m}(\theta, \xi)\,.
\eea
So, at this point the thin-shell approximation is usually invoked and this implicitly assumes continuous functions in Fourier space. That means
\be
\sum_{\qv \in k}\rightarrow \int_{k} \frac{d^3q}{k_f^3}\,,
\ee
and eq.~\ref{e:Bexp} and \ref{e:Blm} to be exact, so that
\bea
\langle\hat B_{\ell m}(k_1, k_2, k_3)\rangle 
& = & \frac{k_f^3}{N_B(k_1, k_2, k_3)}\int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\delta_D(\qv_{123})\,B(\qv_1,\qv_2,\qv_3) Y_{\ell m}(\theta, \xi)\nn\\
& = & \frac{k_f^3}{N_B(k_1, k_2, k_3)}\int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\delta_D(\qv_{123})\nn
\\
& & \times\sum_{\ell',m'}B_{\ell' m'}(q_1,q_2,q_3) Y_{\ell' m'}(\theta, \xi) Y_{\ell m}(\theta, \xi)\nn\\
& \stackrel{k_i\gg \Delta k}{\simeq} & \sum_{\ell',m'}B_{\ell' m'}(k_1,k_2,k_3)\frac{k_f^3}{N_B(k_1, k_2, k_3)}\int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\delta_D(\qv_{123})\nn\\
& & 
\times Y_{\ell' m'}(\theta, \xi) Y_{\ell m}(\theta, \xi)\nn\\
& \simeq & \sum_{\ell',m'}B_{\ell' m'}(k_1,k_2,k_3)\frac{k_f^3}{N_B(k_1, k_2, k_3)}\int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\delta_D(\qv_{123})
\nn\\ & & 
\times\delta_{\ell\ell'}\delta_{m m'}\nn\\
& = & B_{\ell m}(k_1,k_2,k_3)\frac{k_f^3}{N_B(k_1, k_2, k_3)}\int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\delta_D(\qv_{123})\nn\\
& = & B_{\ell m}(k_1,k_2,k_3)
\,,
\eea
confirming the estimator to be unbiased. We clearly assumed 
\bea
N_B(k_1, k_2, k_3) 
& \simeq & \int_{k_1} \frac{d^3q_1}{k_f^3}\int_{k_2} \frac{d^3q_2}{k_f^3}\int_{k_3} \frac{d^3q_3}{k_f^3}\,k_f^3\,\delta_D(\qv_{123})\,.
\eea
\emi{All this was just to check the normalisation ... sorry I have to stop here now.} 

Let's take the case of the power spectrum instead, and suppose we are in 2D with the LOS on the y-axis and a Kaiser model. The estimator of the power spectrum multipoles is 
\be
\hat P_{\ell}(k) = \frac{1}{V}\frac{1}{N_P(k)}\sum_{\qv \in k}\,|\delta(\qv)|^2{\mathcal L}_\ell(\mu)\,,
\ee
with $\mu=\cos\theta$, $\theta$ being the angle between $\qv$ and the y-axis and where $N_P(k)=\sum_{\qv\in k}$. 
Suppose we only look at the first $k$-bin centered at $k_f$ of size $\Delta k=k_f$. The wavenumbers in the bin are $(\pm 1,0)k_f, (0, \pm 1)k_f$ and $(\pm 1,\pm 1)k_f$ with $N_P(k_f)=8$. The corresponding values of $\mu$ are $\pm 0$, $\pm 1$ and $\pm 1/\sqrt{2}$ (these last with multiplicity equal to 2). The estimated first bin of the power spectrum is therefore, in average,
\bea
\label{e:Plest}
\langle\hat P_{\ell}(k_f)\rangle &  = &  \frac{1}{N_P(k)}\sum_{\qv \in k}\,P(\qv)\,{\mathcal L}_\ell(\mu)\nn\\
&  = &  \frac{1}{N_P(k)}\left[2\,P(k_f,0)\,{\mathcal L}_\ell(0)
+2\,P(k_f,1)\,{\mathcal L}_\ell(1)
+4\,P(\sqrt{2}\,k_f,1/\sqrt{2})\,{\mathcal L}_\ell(1/\sqrt{2})\right]\,,
\eea
where I assumed $P(k,\mu)$ to be even in $\mu$ so that I can consider only even Legendre polynomials. 

Now, the binned, linear theoretical prediction for the multipole, given a model for the 2D power spectrum $P^{th}(k\mu)$, is given by
\be
\label{e:Plbinned}
P_{\ell}^{th, binned}(k) = \frac{1}{N_P(k)}\sum_{\qv \in k}\,P^{th}(\qv) {\mathcal L}_\ell(\mu)\,,
\ee
and this can be expanded to get exactly the discrete expression above. 

Suppose instead that I consider the {\em continuous} expansion in Legendre polinomials given by
\be
\widetilde{P}^{th}(\qv)=\sum_\ell \widetilde{P}_\ell^{th}(q)\,{\mathcal L}_\ell(\mu)
\ee
where
\be
\widetilde{P}_\ell^{th}(q)=\int d\mu\,\widetilde{P}^{th}(q,\mu)\,{\mathcal L}_\ell(\mu)\,,
\ee
ad I write the binned prediction for the $P_\ell(k)$ in terms of the $P_\ell^{th}(k)$ defined here. I have
\bea
\widetilde{P}_{\ell}^{th, binned}(k_f) & = &  \frac{1}{N_P(k)}\sum_{\qv \in k_f}\,\sum_{\ell'} \widetilde{P}_{\ell'}^{th}(q)\,{\mathcal L}_{\ell'}(\mu) {\mathcal L}_\ell(\mu)\nn\\
 & = & \frac{1}{N_P(k)}\sum_{\ell'}\,\sum_{\qv \in k_f}\, \widetilde{P}_{\ell'}^{th}(q)\,{\mathcal L}_{\ell'}(\mu) {\mathcal L}_\ell(\mu)\nn\\
 & = & \frac{1}{N_P(k)}\sum_{\ell'}\,\left[2\,\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(0) {\mathcal L}_\ell(0)+
 2\,\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(1) {\mathcal L}_\ell(1)+\right.\nn\\ & & 
\left.+ 4\,\widetilde{P}_{\ell'}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{\ell'}(1/\sqrt{2}) {\mathcal L}_\ell(1/\sqrt{2})\right]\,,
\eea 
but clearly this does not coincide with eq.~\ref{e:Plest} since quantities like  $\widetilde{P}_{\ell'}^{th}(k_f)$ are integrals over {\em all} the values of $-1\le \mu\le 1$ while in a box I only have 4 possible values for the first bin.

Let's take the linear Kaiser model to be the truth,
\be
P(q,\mu)=P^{th}(q,\mu)=(1+f\,\mu^2)^2\,P_L(q)
\ee
Then the first bin of the estimated quadrupole will be  
\bea
\langle\hat P_{2}(k_f)\rangle 
&  = &  \frac{1}{N_P(k_f)}\left[2\,P(k_f,0)\,{\mathcal L}_\ell(0)
+2\,P(k_f,1)\,{\mathcal L}_\ell(1)
+4\,P(\sqrt{2}\,k_f,1/\sqrt{2})\,{\mathcal L}_\ell(1/\sqrt{2})\right]\nn\\
&  = &  \frac{1}{N_P(k_f)}\left\{2\,P_L(k_f)\,\left[\,{\mathcal L}_2(0)+(1+f)^2\,\,{\mathcal L}_2(1)\right]
+4\,P_L(\sqrt{2}\,k_f)\,(1+f/2)^2\,{\mathcal L}_2(1/\sqrt{2})\right\}\nn\\
&  = &  \frac{1}{N_P(k_f)}\left\{2\,P_L(k_f)\,\left[-\frac12+(1+f)^2\right]
+4\,P_L(\sqrt{2}\,k_f)\,(1+f/2)^2\,\frac14\right\}\nn\\
&  = &  \frac{1}{N_P(k_f)}\left\{P_L(k_f)\,\left[-1+2\,(1+f)^2\right]
+P_L(\sqrt{2}\,k_f)\,(1+f/2)^2\right\}\nn\\
&  = &  \frac{1}{N_P(k_f)}\left\{P_L(k_f)\,\left[1+4\,f+2\,f^2\right]
+\frac14\,P_L(\sqrt{2}\,k_f)\,(2+f)^2\right\}\,.
\label{e:example}
\eea
By definition, I can get the same expression from eq.~\ref{e:Plbinned}. But also
\bea
\widetilde{P}_{2}^{th, binned}(k_f) 
 & = & \frac{1}{N_P(k_f)}\sum_{\ell'}\,\left[2\,\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(0) {\mathcal L}_2(0)+
 2\,\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(1) {\mathcal L}_2(1)+\right.\nn\\ 
 & & 
\left.+ 4\,\widetilde{P}_{\ell'}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{\ell'}(1/\sqrt{2}) {\mathcal L}_2(1/\sqrt{2})\right.\nn\\
& = & \frac{1}{N_P(k_f)}\sum_{\ell'}\,\left[-\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(0) +
 2\,\widetilde{P}_{\ell'}^{th}(k_f)\,{\mathcal L}_{\ell'}(1)+ \widetilde{P}_{\ell'}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{\ell'}(1/\sqrt{2})\right]\,,
\eea 
where 
\bea
\widetilde{P}_{0}^{th}(k_f) & = & \left(1+\frac23\,f+\frac15\,f^2\right)P_L(k_f)\\
\widetilde{P}_{2}^{th}(k_f) & = & \left(\frac43\,f+\frac47\,f^2\right)P_L(k_f)\\
\widetilde{P}_{4}^{th}(k_f) & = & \frac8{35}\,P_L(k_f)\\
\eea
so that
\bea
\widetilde{P}_{2}^{th, binned}(k_f) 
& = & \frac{1}{N_P(k_f)}\left\{
\left[-\widetilde{P}_{0}^{th}(k_f)\,{\mathcal L}_{0}(0) +
 2\,\widetilde{P}_{0}^{th}(k_f)\,{\mathcal L}_{0}(1)+ \widetilde{P}_{0}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{0}(1/\sqrt{2})\right]+
 \right.\nn\\ & & \left.
 \left[-\widetilde{P}_{2}^{th}(k_f)\,{\mathcal L}_{2}(0) +
 2\,\widetilde{P}_{2}^{th}(k_f)\,{\mathcal L}_{2}(1)+ \widetilde{P}_{2}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{2}(1/\sqrt{2})\right]+
 \right.\nn\\ & & \left.
 \left[-\widetilde{P}_{4}^{th}(k_f)\,{\mathcal L}_{4}(0) +
 2\,\widetilde{P}_{4}^{th}(k_f)\,{\mathcal L}_{4}(1)+ \widetilde{P}_{4}^{th}(\sqrt{2}\,k_f)\,{\mathcal L}_{4}(1/\sqrt{2})\right]
 \right\}\nn\\
 & = & \frac{1}{N_P(k_f)}\left\{
\left[-\widetilde{P}_{0}^{th}(k_f) +
 2\,\widetilde{P}_{0}^{th}(k_f)+ \widetilde{P}_{0}^{th}(\sqrt{2}\,k_f)\right]+
 \right.\nn\\ & & \left.
 \left[\frac12\widetilde{P}_{2}^{th}(k_f) +
 2\,\widetilde{P}_{2}^{th}(k_f)+ \frac14\,\widetilde{P}_{2}^{th}(\sqrt{2}\,k_f)\right]+
 \right.\nn\\ & & \left.
 \left[-\frac38\,\widetilde{P}_{4}^{th}(k_f) +
 2\,\widetilde{P}_{4}^{th}(k_f)-\frac{13}{32} \widetilde{P}_{4}^{th}(\sqrt{2}\,k_f)\right]
 \right\}\nn\\
 & = & \frac{1}{N_P(k_f)}\left\{
\left[\widetilde{P}_{0}^{th}(k_f) + \widetilde{P}_{0}^{th}(\sqrt{2}\,k_f)\right]+
 \right.\nn\\ & & \left.
 \left[\frac52\widetilde{P}_{2}^{th}(k_f) +
  \frac14\,\widetilde{P}_{2}^{th}(\sqrt{2}\,k_f)\right]+
 \right.\nn\\ & & \left.
 \left[\frac{13}{8}\,\widetilde{P}_{4}^{th}(k_f) -\frac{13}{32} \widetilde{P}_{4}^{th}(\sqrt{2}\,k_f)\right]
 \right\}\nn\\
  & = & \frac{1}{N_P(k_f)}\left[(1+4\,f+2\,f^2)\,P_L(k_f) +\frac14(2+f)^2\,P_L(\sqrt{2}\,k_f)\right]\,,
\eea
which is exactly as eq.~\ref{e:example}. OK ... I am 90\% convinced, but clearly this should be derived in full generality and now it's too late ...

-----
We first evaluate the prediction on the effective $k$-s using continuous integration over angles and show that, for the bispectrum multipoles, this kind of prediction is not accurate enough if one does not properly bin the model.



%%% OLD STUFF

%\subsection{Binning effects}

% In the case of the monopole, where the legendre polynomial of order zero is just a constant,
% $Y_0^0(\theta, \xi)=\frac{1}{2}\sqrt{\frac{1}{\pi}}$, equation 3 can be written as a sum in orders of $\mu$:
% \be
% \begin{aligned}
%     \mathcal{O}[\mu^0]&=\sqrt{\frac{1}{\pi}}\Big[b^2_1\Big(\frac{b_2}{2}+b_1F_2(k_1, k_2; k_3)+b_{\mathcal{G}_2}S(k_1, k_2; k_3)\Big)\mathcal{I}_{000}\Big]P(k_1)P(k_2)\\
%     \mathcal{O}[\mu^2] &=\sqrt{\frac{1}{\pi}}\Big[b_1 f \Big(\frac{b_2}{2}+b_1F_2(k_1, k_2; k_3)+b_{\mathcal{G}_2}S(k_1, k_2; k_3)\Big)(\mathcal{I}_{200}+\mathcal{I}_{020}) +\\
%     &\qquad\qquad + b_1^2f G_2(k_1, k_2; k_3)\mathcal{I}_{002}-\frac{b_1^3 f}{2}\Big(\frac{k_3}{k_1}\mathcal{I}_{101}+\frac{k_3}{k_2}\mathcal{I}_{011}\Big)\Big]P(k_1)P(k_2)\\
%     \mathcal{O}[\mu^4] & =\sqrt{\frac{1}{\pi}}\Big[f^2 \Big(\frac{b_2}{2}+b_1 F_2(k_1, k_2; k_3)+b_{\mathcal{G}_2}S(k_1, k_2; k_3)\Big)\mathcal{I}_{220}+b_1 f^2 G_2(k_1, k_2; k_3) (\mathcal{I}_{202}+\mathcal{I}_{022}) +\\
%     &\qquad\qquad -\frac{b_1^2f^2}{2}\Big(\frac{k_3}{k_1}(\mathcal{I}_{301}+2\mathcal{I}_{121}) + \frac{k_3}{k_2}(\mathcal{I}_{031}+2\mathcal{I}_{211})\Big)\Big]P(k_1)P(k_2) \\ 
%     \mathcal{O}[\mu^6] &=\sqrt{\frac{1}{\pi}}\Big[f^3 G_2(k_1, k_2; k_3)\mathcal{I}_{222}-\frac{b_1 f^3}{2}\Big(\frac{k_3}{k_1}(\mathcal{I}_{141}+2\mathcal{I}_{321}) + \frac{k_3}{k_2}(\mathcal{I}_{411}+2\mathcal{I}_{231})\Big)\Big]P(k_1)P(k_2) \\
%     \mathcal{O}[\mu^8] &=-\sqrt{\frac{1}{\pi}}\Big[\frac{f^4}{2}\Big(\frac{k_3}{k_1}\mathcal{I}_{341} + \frac{k_3}{k_2}\mathcal{I}_{431}\Big)\Big]P(k_1)P(k_2)
% \end{aligned}
% \ee
% Adding the cyclic contributions, one obtains the following:
% \be
% \begin{aligned}
%     \mathcal{O}[\mu^0]&=\sqrt{\frac{1}{\pi}}\Big\{\frac{b^2_1 b_2}{2}(P_1 P_2+P_1 P_3+P_2 P_3)+b_1^3 [F_{2,12}P_1 P_2+F_{2,13}P_1 P_3+F_{2,23}P_2 P_3]\\
%     & \qquad\qquad\qquad+b^2_1 b_{\mathcal{G}_2}[S_{2,12}P_1 P_2+S_{2,13}P_1 P_3+S_{2,23}P_2 P_3]\Big\}\mathcal{I}_{000}\\
%     \mathcal{O}[\mu^2] &=\sqrt{\frac{1}{\pi}} \Big\{\frac{b_1 b_2 f}{2}\Big[(\mathcal{I}_{200}+\mathcal{I}_{020})P_1 P_2+ (\mathcal{I}_{200}+\mathcal{I}_{002})P_1 P_3+
%     (\mathcal{I}_{020}+\mathcal{I}_{002})P_2 P_3\Big]+\\
%     &\qquad\qquad\qquad + b_1^2 f\Big[F_{2, 12}(\mathcal{I}_{200}+\mathcal{I}_{020})P_1 P_2+ F_{2, 13}(\mathcal{I}_{200}+\mathcal{I}_{002})P_1 P_3+ F_{2,23}(\mathcal{I}_{020}+\mathcal{I}_{002})P_2 P_3\Big]+\\
%     & \qquad\qquad\qquad + b_1 b_{\mathcal{G}_2}f\Big[S_{2, 12}(\mathcal{I}_{200}+\mathcal{I}_{020})P_1 P_2+S_{2, 13}(\mathcal{I}_{200}+\mathcal{I}_{002})P_1 P_3+S_{2, 23}(\mathcal{I}_{020}+\mathcal{I}_{002})P_2 P_3 \Big]+\\
%     & \qquad\qquad\qquad+ b_1^2f\Big[G_{2,12}\mathcal{I}_{002}P_1 P_2+G_{2,13}\mathcal{I}_{020}P_1 P_3+G_{2,23}\mathcal{I}_{200}P_2 P_3\Big]+ \\
%     &\qquad\qquad\qquad -\frac{b_1^3 f}{2}\Big[\Big(\frac{k_3}{k_1}\mathcal{I}_{101}+\frac{k_3}{k_2}\mathcal{I}_{011}\Big)P_1 P_2 +\Big(\frac{k_2}{k_1}\mathcal{I}_{110}+\frac{k_2}{k_3}\mathcal{I}_{011}\Big)P_1 P_3+\Big(\frac{k_1}{k_2}\mathcal{I}_{110}+\frac{k_1}{k_3}\mathcal{I}_{101}\Big)P_2 P_3\Big]\Big\}\\
%     \mathcal{O}[\mu^4] & =\sqrt{\frac{1}{\pi}} \Big\{\frac{b_2 f^2}{2}\Big[\mathcal{I}_{220}P_1 P_2+ \mathcal{I}_{202}P_1 P_3+\mathcal{I}_{022}P_2 P_3\Big]+b_1 f^2\Big[F_{2, 12}\mathcal{I}_{220}P_1 P_2+ F_{2, 13}\mathcal{I}_{202}P_1 P_3+ F_{2,23}\mathcal{I}_{022}P_2 P_3\Big]+\\
%     &\qquad\qquad\qquad+ b_{\mathcal{G}_2}f^2\Big[S_{2, 12}\mathcal{I}_{220}P_1 P_2+ S_{2,k 13}\mathcal{I}_{202}P_1 P_3+ S_{2,23}\mathcal{I}_{022}P_2 P_3\Big]+\\
%     & \qquad\qquad\qquad+b_1 f^2 \Big[G_{2,12} (\mathcal{I}_{202}+\mathcal{I}_{022})P_1 P_2+ G_{2,13} (\mathcal{I}_{220}+\mathcal{I}_{022})P_1 P_3+ G_{2,23} (\mathcal{I}_{202}+\mathcal{I}_{220})P_2 P_3\Big] +\\
%     &\qquad\qquad\qquad -\frac{b_1^2f^2}{2}\Big[\Big(\frac{k_3}{k_1}(\mathcal{I}_{301}+2\mathcal{I}_{121}) + \frac{k_3}{k_2}(\mathcal{I}_{031}+2\mathcal{I}_{211})\Big)P_1 P_2 +\\ 
%     & \qquad\qquad\qquad\qquad\qquad + \Big(\frac{k_2}{k_1}(\mathcal{I}_{310}+2\mathcal{I}_{112})+\frac{k_2}{k_3}(\mathcal{I}_{013}+2\mathcal{I}_{211})\Big)P_1 P_3+ \\
%     & \qquad\qquad\qquad\qquad\qquad + \Big(\frac{k_1}{k_2}(\mathcal{I}_{130}+2\mathcal{I}_{112})+\frac{k_1}{k_3}(\mathcal{I}_{103}+2\mathcal{I}_{121})\Big)P_2 P_3\Big]\Big\} \\ 
%     \mathcal{O}[\mu^6] &=\sqrt{\frac{1}{\pi}}\Big\{f^3 \Big[G_{2,12}P_1 P_2+ G_{2,13} P_1 P_3+G_{2,23} P_2 P_3\Big]\mathcal{I}_{222}+\\
%     &\qquad\qquad\qquad -\frac{b_1 f^3}{2}\Big[\Big(\frac{k_3}{k_1}(\mathcal{I}_{141}+2\mathcal{I}_{321}) + \frac{k_3}{k_2}(\mathcal{I}_{411}+2\mathcal{I}_{231})\Big)P_1 P_2+\\
%     & \qquad\qquad\qquad\qquad\qquad + \Big(\frac{k_2}{k_1}(\mathcal{I}_{114}+2\mathcal{I}_{312})+\frac{k_2}{k_3}(\mathcal{I}_{411} +2\mathcal{I}_{213})\Big)P_1 P_3+ \\
%     & \qquad\qquad\qquad\qquad\qquad +
%     \Big(\frac{k_1}{k_2}(\mathcal{I}_{114}+ 2\mathcal{I}_{132})+\frac{k_1}{k_3}(\mathcal{I}_{141}+2\mathcal{I}_{123})\Big) P_2 P_3 \Big]\Big\} \\
%     \mathcal{O}[\mu^8] &=-\sqrt{\frac{1}{\pi}}\frac{f^4}{2}\Big\{\Big[\frac{k_3}{k_1}\mathcal{I}_{341} + \frac{k_3}{k_2}\mathcal{I}_{431}\Big] P_1 P_2+\Big[ \frac{k_2}{k_1}\mathcal{I}_{314}+\frac{k_2}{k_3}\mathcal{I}_{413}\Big]P_1 P_3+\Big[\frac{k_1}{k_2}\mathcal{I}_{134}+\frac{k_1}{k_3}\mathcal{I}_{143}\Big]P_2 P_3\Big\}
% \end{aligned}
% \ee
% whith $F_{2,12}=F_2(k_1,k_2;k_3)$, and so on for the mixing kernels. The $\mathcal{I}_{\alpha \beta \gamma}$ terms are numbers that can be computed from the double integral in $\mu_1$ and $\xi$. For the $0$-order contribution in $\mu_i$, $\mathcal{O}[\mu^0]$, one needs only $\mathcal{I}_{000}$:


